A Comparison of Decision Forest Inference Platforms from A Database Perspective

Decision forest, including RandomForest, XGBoost, and LightGBM, is one of the most popular machine learning techniques used in many industrial scenarios, such as credit card fraud detection, ranking, and business intelligence. Because the inference process is usually performance-critical, a number of frameworks were developed and dedicated for decision forest inference, such as ONNX, TreeLite from Amazon, TensorFlow Decision Forest from Google, HummingBird from Microsoft, Nvidia FIL, and lleaves. However, these frameworks are all decoupled with data management frameworks. It is unclear whether in-database inference will improve the overall performance. In addition, these frameworks used different algorithms, optimization techniques, and parallelism models. It is unclear how these implementations will affect the overall performance and how to make design decisions for an in-database inference framework. In this work, we investigated the above questions by comprehensively comparing the end-to-end performance of the aforementioned inference frameworks and netsDB, an in-database inference framework we implemented. Through this study, we identified that netsDB is best suited for handling small-scale models on large-scale datasets and all-scale models on small-scale datasets, for which it achieved up to hundreds of times of speedup. In addition, the relation-centric representation we proposed significantly improved netsDB's performance in handling large-scale models, while the model reuse optimization we proposed further improved netsDB's performance in handling small-scale datasets.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

==> optimization.tex <==
%\section{Optimization of Decision Tree in RDBMS}
%\label{sec:rdbms-approaches}
%\subsection{Overhead Analysis and Problem Identification}

%\subsubsection{UDF-based Approach}

%\subsubsection{Join-based Approach}

%\subsubsection{Driver-based Approach}

%\subsection{On-Demand Model Materialization for the UDF-based Approach} 

%The overhead analysis showed that for the dynamic UDF approach, a lot of time is spent in initializing the UDF local variables based on the model specification file. Although static UDF doesn't have such problem, manually programming an ensemble model into a UDF is tedious and different ensemble tree workloads can hardly share any code or optimization techniques with each other, because each UDF is programmed separately by its application developer. 

%To address these issues, we propose to improve the dynamic UDF approach by providing a model materialization mechanism, so that the user can first register a model by supplying the model specification file, which is used to deserialize the model as an ensemble tree object, which will be cached in memory. The model registration process returns a model ID to the user. 
%The RDBMS provides a generic decision tree UDF that takes a batch of feature vectors and a ensemble tree model ID as inputs. Then, the UDF uses the model ID to locate and access the model object in memory directly and runs the model's predict function over the input feature vectors and  output the final batch of predicted labels correspondingly. 

%By applying the model materialization approach, we saved the time for deserializing the ensemble model object for each inference query. Instead, all inference queries of the same model can directly access the materialized model object from memory.

%While the idea is quite straightforward, the implementation could be challenging depending on the database system architecture. If each job is launched in a separate process at runtime, like Spark, it is difficult to make the materialized model in memory visible and reusable to all jobs, unless leverging external caching system such as Alluxio~\cite{}. 

%We mainly implement the idea on our netsDB system, which is a  distributed object-oriented relational database built on top of our previous work in PlinyCompute~\cite{zou2018plinycompute, zou2019pangea, DBLP:journals/pvldb/ZouDBIYJJ21}. Each worker in the netsDB system has one parent front-end process for caching data and a long-living child backend process for executing various user queries. The front-end process and the backend process share the buffer pool memory via the anonymous mmap system call. We thus have two options: (1) Storing the materialized model in the buffer pool, so that it can be managed together with other datasets in a unified way and can be accessed by the backend through shared memory; (2) Storing the materialized model on the heap of the backend process. We choose the second option because accessing shared memory requires another layer of indirection, for example, the shared memory is usually mapped to different addresses in the parent process and the child process, thus we need first obtain the offset in the shared memory and then convert it to the pointer address for dereferencing.

%Another complexity is in the translation of the model ID to the pointer address of the ensemble in the UDF. The UDF is defined by users or library developers, and the system runtime details such as memory addressing and caching should be transparent to them. To address the problem, we developed a lightweight file-backed metadata store, from which the UDF can query the pointer address using the model ID.

%\subsection{Dynamic Model Materialization for the Join-based Approach}
%As explained in the overhead analysis, deserializing the model dataset to an array of tree objects in memory so that each tree object is ready to be paired with each input feature vector, becomes the major overhead for the join operation, which is actually a cross-product operation. 

%Again, we find it is hard to implement this idea in a system like Spark, because Spark is mainly a computation framework instead of a data storage framework, and the data cache is not visible across jobs.
%Therefore, we implement the idea also on our netsDB system, which integrates the computation with storage just like traditional RDBMS.

%Different from UDF approach, the model materialization for the Join-based approach is not required to be initiated by the user. Instead it is automatically conducted by the join operation, transparent to the user. Therefore, it further reduce the burden from the application/library developers' side. 

%To achieve this, we modified netsDB's job scheduler to record the identifiers of historical input datasets for each join operation.  The scheduler will predict the probability that a dataset may be reused for a join algorithm based on the historical information. The intuition is that if the scheduler detects that a dataset is repeatedly joined with other datasets, and the dataset has not been changed at all through these repeated processing, the dataset will probably be reused for join in the future. There are many mechanisms to estimate this reuse probability~\cite{}, including ... We propose a ..., because...

%Once the predicted reuse probability is higher than a threshold, the dataset will be deserialized and materialized in memory for future use. The materialized data will be associated with the ID of join algorithm. That's Because each different join algorithm has different requirements for the materialization. For example, hash partition join requires to materialize the dataset into a hash map, sort merge join requires to materialize the dataset into a sorted list, and nested loop join requires to materialize the dataset into a list. A dataset can be materialized into different forms to benefit different algorithms, though that will incur additional storage costs. We will discuss this issue in Sec.~\ref{sec:caching}.

%Next time when the dataset needs to be joined with another dataset, and the query optimizer chooses the same join algorithm, the scheduler will skip the materialization stage, and directly notify the join operator the location of the materialized data in the backend process.


%\subsection{Automatic Compilation and Code-Generation of Static UDFs}
%Another optimization technique that we explored is to automatically generate prediction code in form of LLVM intermediate representation (IR) from the model specification file using LLVM. The LLVM IR will be used to create a static UDF, which will parse the IR to extract the prediction function at runtime to run inferences on the input feature vectors.

%This will significantly improve the productivity of the static UDF approach. We implemented three different algorithms for the generated code: 

%\vspace{5pt}
%\noindent
%(1) IF-THEN-ELSE. We translate the input model specification file 

%\vspace{5pt}
%\noindent
%(2) PRED


%\vspace{5pt}
%\noindent
%(3) VPRED





%\subsection{Further Discussions}
%\subsubsection{Caching}
%\label{sec:caching}
%Decision tree models tend take less storage space compared to deep neural network models. For example, a large-scale ensemble tree model that has at most $1024$ trees with each having a depth of $10$ ($2048$ tree nodes), takes only about $16$ megabytes' storage space, if each node minimally contains three attributes including the feature id ($2$ bytes), the threshold/label ($4$ bytes), and the node id/offset ($2$ bytes). Therefore, the storage of ensemble decision tree models may not be a severe issue for high-end servers in cloud data centers. 

%If the environment is memory-bound, we advocate to materialize the model in the front-end process, and allow the backend to access the materialized data through the shared memory. Although this way incurs overheads for translating the offset in shared memory to the pointer address in the backend process, all datasets, materialized or not materialized, can be managed in the buffer pool under unified page replacement policy.



%\subsubsection{Model Updates}
%Once a model gets removed or updated, all materialized versions of the model need to be removed and updated accordingly. We considered to accelerate the updating process by computing a hash signature for each tree~\cite{wang2015schema}, only trees that are changed need to be updated. However, it turns out that the additional overheads for computing the hash signatures for each tree overweights the overheads for updating.



==> relatedworks.tex <==





